Efficient View Synthesis with Neural Radiance Distribution Field

Recent work on Neural Radiance Fields (NeRF) has demonstrated significant advances in high-quality view synthesis. A major limitation of NeRF is its low rendering efficiency due to the need for multiple network forwardings to render a single pixel. Existing methods to improve NeRF either reduce the number of required samples or optimize the implementation to accelerate the network forwarding. Despite these efforts, the problem of multiple sampling persists due to the intrinsic representation of radiance fields. In contrast, Neural Light Fields (NeLF) reduce the computation cost of NeRF by querying only one single network forwarding per pixel. To achieve a close visual quality to NeRF, existing NeLF methods require significantly larger network capacities which limits their rendering efficiency in practice. In this work, we propose a new representation called Neural Radiance Distribution Field (NeRDF) that targets efficient view synthesis in real-time. Specifically, we use a small network similar to NeRF while preserving the rendering speed with a single network forwarding per pixel as in NeLF. The key is to model the radiance distribution along each ray with frequency basis and predict frequency weights using the network. Pixel values are then computed via volume rendering on radiance distributions. Experiments show that our proposed method offers a better trade-off among speed, quality, and network size than existing methods: we achieve a ~254x speed-up over NeRF with similar network size, with only a marginal performance decline. Our project page is at yushuang-wu.github.io/NeRDF.

==> figures/fig_model_compare_bubble.tex <==
\begin{figure}[tb] 
    \centering
    \makebox[0.45\linewidth]{\scriptsize (a) Speed - PSNR - Model size}
    \makebox[0.45\linewidth]{\scriptsize (b) FLOPs - PSNR - Model size}
    \\
    \includegraphics[width=0.45\linewidth]{images/bubble_chart_speed.png}
    \includegraphics[width=0.45\linewidth]{images/bubble_chart_flops.png}
    \caption{Visualization of Speed(FLOPs)-PSNR-Size for efficient view synthesis methods.
             Bubble sizes indicates model size. (a) Our method (marked in red) is the only method that achieves real-time speed while preserves plausible quality.
             (b) Our method (marked in red) has the smallest MFLOPs as well as model size while preserves plausible quality.}
    \label{fig:model_compare_bubble}
\end{figure}

==> figures/fig_network.tex <==
\begin{figure*}[!ht] 
    \centering
    \includegraphics[width=0.8\linewidth]{images/network.pdf}
    \caption{The network structure for NeRDF with 8 layers and 8 mix-of-gaussians modes.}
    \label{fig:network_structure}
    \vspace{-2mm}
\end{figure*}

==> figures/fig_psnr_curve.tex <==
\begin{figure}[tb] 
    \centering
    \includegraphics[width=0.42\textwidth]{images/psnr_curve.png}
    \caption{Trade-off curve between PSNR and speed-up ratio of different efficient view synthesis methods. Our method (the blue curve) has a significant better trade-off than other methods.}
    \label{fig:psnr_curve}
\end{figure}

==> figures/fig_teaser.tex <==
\begin{figure*}[ht]
\centering
    \captionsetup{type=figure}
    \makebox[0.23\linewidth]{\small PSNR = 26.80, \textcolor{red}{$\sim$0.2 FPS}}
    \makebox[0.23\linewidth]{\small PSNR = 26.87, \textcolor{red}{$\sim$3.6 FPS}}    
    \makebox[0.23\linewidth]{\small \textcolor{red}{PSNR = 21.10}, $\sim$15.6 FPS}
    \makebox[0.23\linewidth]{\small \color[HTML]{239B56}PSNR = 25.69, $\sim$23.4 FPS}
    \\
    \includegraphics[width=0.23\linewidth]{images/teaser_nerf.png}
    \includegraphics[width=0.23\linewidth]{images/teaser_r2l_d88.png}
    \includegraphics[width=0.23\linewidth]{images/teaser_r2l_d8.png}
    \includegraphics[width=0.23\linewidth]{images/teaser_ours.png}
    \\
    \makebox[0.23\linewidth]{\small NeRF, 8-layer MLP}   
    \makebox[0.23\linewidth]{\small R2L, \textcolor{red}{88-layer MLP}}    
    \makebox[0.23\linewidth]{\small R2L, 16-layer MLP}
    \makebox[0.23\linewidth]{\small NeRDF (Ours), \color[HTML]{239B56}8-layer MLP}
    \\
    \caption{State-of-the-art view synthesis methods (column 1-3) exhibits an impossible trinity of visual quality, fast rendering speed, and low cost. Our method (rightmost) breaks this trinity and enables real-time efficient view synthesis with low cost.} 
    \label{fig:teaser_compare}
\end{figure*}
%\scriptsize

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> make_files.tex <==
mkdir images tables figures
touch 0_main.tex 1_abstract.tex 2_intro.tex 3_relatedwork.tex 4_method.tex 5_experiments.tex 6_conclusions.tex 7_supp.tex


==> tables/ablation_distillation.tex <==
\begin{table}[tb]\centering
    \caption{The impact of adding distillation constraint to NeRDF. VD stands for volume density constraint and CD stands for radiance color constraint. All NeRDFs is trained with 8-layers with 8 mixture-of-gaussians modes.}
    \label{tab:ablation_distillation}
    \resizebox{0.75\linewidth}{!}{
    \large
    \begin{tabular}{*{10}{c}}
        \toprule
        Variants & Train. PSNR & Test. PSNR \\
        \midrule
        NeRDF           & 22.83 & 23.65 \\
        NeRDF + VD      & 23.02 & 23.93 \\
        NeRDF + VD + CD & 23.04 & 23.94 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/ablation_netwidth.tex <==
\begin{table}[tb]\centering
    \caption{The synthesis quality and rendering speed of using different network width with an MLP with 8 layers.}
    \label{tab:ablation_netwidth}
    \resizebox{0.9\linewidth}{!}{ \small
    \begin{tabular}{*1{l} *5{c}}
        \toprule
        Width      & 256 & 320 & 384 & 448 & 512 \\
        \midrule
        PSNR(dB)   & 25.15 & 25.43 & 25.69 & 25.80 & 25.97 \\
        % \midrule
        FPS        & 31.06 & 24.27 & 21.18 & 16.61 & 14.66 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
\end{table}

==> tables/ablation_netwidth_384.tex <==
\begin{table}[tb]\centering
    \caption{The synthesis quality (PSNR, dB) comparison between R2L (a) and different variants of NeRDF (b,c,d) on FERN and FLOWER, with network width 384.}
    \label{tab:ablation_384}
    \resizebox{1.0\linewidth}{!}{
    \large
    \begin{tabular}{*{6}{c}}
        \toprule
        Idx & Distribution & ~~~OVS~~~ & ~~~VDC~~~ & ~~~FERN~~~ & ~FLOWER~ \\
        \midrule
        (a) &            &            &            & 23.45 & 23.33\\
        (b) & \checkmark &            &            & 25.58 & 24.85\\
        % (c) &            & \checkmark &            & 24.91 & 26.41\\
        (c) & \checkmark & \checkmark &            & 25.65 & 27.74\\
        (d) & \checkmark & \checkmark & \checkmark & \textbf{25.69} & \textbf{27.85}\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table}

==> tables/ablation_numGauss.tex <==
% \begin{table}[tb]\centering
%     \caption{The impact of the number of gaussian modes $K$ for an 8-layer NeRDF.
%              Our method is robust to the selection of $K$ from 8 to 32.}
%     \label{tab:ablation_numGauss}
%     \resizebox{0.8\linewidth}{!}{ \small
%     \begin{tabular}{*{6}{c}}
%         \toprule
%          % & 2 & $K$=4 &  $K$=8 & $K$=16 & $K$=32 \\
%         $K$= & 2 & 4 & 8 & 16 & 32 \\
%         \midrule
%         PSNR$\uparrow$  & 23.54 & 24.23 & 24.29 & 24.30 & 24.26 \\
%         SSIM$\downarrow$& 0.970 & 0.974 & 0.974 & 0.974 & 0.974 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}
\begin{table}[tb]\centering
    \caption{The synthesis quality comparison of using trigonometric functions and GMM to approximate the radiance distribution and the impact of the number of frequencies/components used.}
    \label{tab:ablation_K_GMM}
    \resizebox{0.9\linewidth}{!}{ \small
    \begin{tabular}{*1{l} *5{c}}
        \toprule
        TrigF: $K$ & 4 & 8 & 12 & 16 & 24 \\
        \hline
        PSNR(dB)   & 25.63 & 25.64 & \textbf{25.69} & 25.66 & 25.67 \\
        \midrule
        GMM: $K'$ & 2 & 4 & 8 & 16 & 32 \\
        \hline
        PSNR(dB)  & 24.88 & 25.57 & \textbf{25.63} & \textbf{25.63} & 25.60 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table}

==> tables/ablation_online.tex <==
\begin{table}[tb]\centering
    \caption{The effect of using online view sampling to generate pseudo-data from the teacher NeRF.
             The ``offline" refers to the same strategy used in R2L~\cite{wang2022r2l}.}
    \label{tab:ablation_online}
    \resizebox{0.75\linewidth}{!}{
    \large
    \begin{tabular}{*{10}{c}}
        \toprule
        Variants & Train. PSNR & Test. PSNR \\
        \midrule
        NeRDF (offline)     & 23.04 & 23.94 \\
        NeRDF (online)      & 26.45 & 24.29 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/ablation_radiance_distribution.tex <==
\begin{table}[tb]\centering
    \caption{The impact of using radiance distribution. D and G denotes network depth and number of gaussian modes respectively.}
    \label{tab:ablation_radiance_distribution}
    \resizebox{0.9\linewidth}{!}{
    \large
    \begin{tabular}{*{4}{c}}
        \toprule
        Method & NeRDF (D8-G8) &  NeLF (D8) & NeLF  (D16) \\
        \midrule
        PSNR$\uparrow$ & 24.29 & 21.17 & 23.21 \\
        SSIM$\uparrow$ & 0.974 & 0.954 & 0.970 \\
        \bottomrule
    \end{tabular}    
%    \begin{tabular}{*{4}{c}}
%        \toprule
%        Variant & PSNR$\uparrow$ &  %SSIM$\uparrow$ &  LPIPS$\downarrow$ \\
%        \midrule
%        NeRDF (D8-G8) & 24.29 & 0.974 & 0.308 \\
%        NeLF  (D8)    & 21.10 & \textcolor{red}{0.925} & \textcolor{red}{0.356} \\
%        NeLF  (D16)   & \textcolor{red}{21.50} & \textcolor{red}{0.928} & \textcolor{red}{0.371} \\
%        \bottomrule
%    \end{tabular}
    }
\end{table}

==> tables/ablation_sample.tex <==
\begin{table}[!ht]\centering
    \caption{The PSNR(dB) of NeRDF  when using different number of sampling points for neural rendering in training (Train-$n$) and inference (Infer-$n$), with $n \in \{16, 32, 64, 128\}$.}% The inference time is measured under the resolution of 504$\times$378.}
    \label{tab:gaussian_sample}
    \resizebox{0.95\linewidth}{!}{ \small
    \begin{tabular}{*{5}{c}}
        \toprule
           & Infer-16 & Infer-32 & Infer-64 & Infer-128\\
        \midrule
        Train-16~~  & 25.62 & 25.62 & 25.62 & 25.62  \\
        Train-32~~  & 25.65 & 25.66 & 25.66 & 25.66  \\
        Train-64~~  & 25.50 & 25.65 & 25.69 & 25.67  \\
        Train-128   & 24.96 & 25.65 & 25.70 & 25.70  \\
        \midrule
        Infer. time (ms) & 1.2 & 1.6 & 2.5 & 3.8 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
\end{table}

==> tables/ablation_speed_ratio.tex <==
\begin{table}[!ht]\centering
    \caption{The speed-up ratio (compared to NeRF~\cite{mildenhall2020_nerf_eccv20}) of the proposed NeRDF on different GPU devices.}
    \label{tab:speed-up-ratio}
    \resizebox{0.85\linewidth}{!}{ \small
    \begin{tabular}{*{4}{c}}
        \toprule
        GPU Type & RTX3090 & ~~V100~~ & ~~A100~~ \\
        \midrule
        Speed-up ratio ($\times$) & 135.2 & 137.7 & 162.3  \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/breakdown.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
    \centering
    \caption{Per-scene breakdown results on the Real Forward Facing dataset of rendering an image of resolution 504$\times$378.}
    \label{tab:breakdown}
    \resizebox{1.0\linewidth}{!}{    
    \begin{tabular}{lccccccccccc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Memory $\downarrow$} & \multirow{2}{*}{~~~~~FPS $\uparrow$~~~~~} & \multicolumn{9}{c}{PSNR (dB)} \\ 
    \cmidrule{4-12} 
                   & (MB) & (RTX 3090, PyTorch)          & Fern  & Flower & Fortress & Horns & Leaves & Orchids & Room  & T-Rex & Average\\ \midrule
    Teacher NeRF   & ~~3.8 & ~~0.17  & 26.81 & 28.44  & 31.68    & 29.62 & 22.38  & 21.37   & 33.13 & 28.61 & 27.75 \\ 
    \midrule
    R2L-8          & ~~2.2 & 33.67   & 22.61 & 22.01  & 25.85    & 22.02 & 18.15  & 17.30   & 26.37 & 22.06 & 22.05 \\
    R2L-16         & ~~4.6 & 20.12   & 24.57 & 25.03  & 28.19    & 24.73 & 20.26  & 19.10   & 29.15 & 24.33 & 24.42 \\
    R2L-32         & ~~8.6 & 11.40   & 25.79 & 26.59  & 29.87    & 26.11 & 21.42  & 20.52   & 30.96 & 25.68 & 25.87 \\
    R2L-48         & 13.0 & ~~7.89   & 26.28 & 26.98  & 30.43    & 26.77 & 21.88  & 21.01   & 31.50 & 26.17 & 26.37 \\
    \midrule
    NeRDF-8        & ~~5.1 & 21.18   & 25.69 & 27.85  & 30.66    & 26.98 & 21.68  & 20.90   & 31.76 & 26.72 & 26.53 \\
    NeRDF-16       & ~~9.6 & 11.88   & 25.93 & 28.18  & 31.01    & 27.44 & 22.03  & 21.09   & 31.98 & 26.96 & 26.82 \\
    NeRDF-32       & 19.0 & ~~6.32   & 25.81 & 28.20  & 30.93    & 27.48 & 22.06  & 21.10   & 32.01 & 26.98 & 26.82 \\
    NeRDF-48       & 28.0 & ~~4.34   & 26.15 & 28.34  & 31.37    & 28.13 & 22.15  & 21.40   & 32.43 & 27.57 & 27.19 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table*}

==> tables/results_llff_efficiency.tex <==
\begin{table*}[t]
    \centering
    \caption{Quantitative comparisons on the Real Forward Facing dataset with a resolution of 504$\times$378. D and G denotes network depth and number of gaussian modes respectively.
             *Results is from AdaNeRF~\cite{kurz2022adanerf} where performances are conducted on a RTX3090 GPU with an optimized TensorRT backend. The top 1/2/3 for each column is denoted as black, orange and blue.}
    \label{tab:res_llff_syn}    
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{@{}lccccccc@{}}
            \toprule
            \multirow{3}{*}{Method}                                     & \multirow{3}{*}{Storage (MB) $\downarrow$} & \multirow{3}{*}{MFLOPs$\downarrow$} & \multicolumn{3}{c}{FPS $\uparrow$}                                                                                                                              & \multirow{3}{*}{Speed-up ($\times$) $\uparrow$} & \multirow{3}{*}{PSNR (dB) $\uparrow$} \\ \cmidrule(lr){4-6}
                                                                        &                               &                         & \begin{tabular}[c]{@{}c@{}}V100\\ (PyTorch)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RTX 3090\\ (PyTorch)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RTX 3090\\ (Optimized)\end{tabular} &                               &                            \\ \midrule
            Teacher NeRF\cite{mildenhall2020_nerf_eccv20}               & 2.4                           & 303.8                   & 0.17                                                     & 0.25                                                         & 1.42*                                                          & 1.0                           & \textcolor{blue}{27.75}                      \\ \midrule
            AutoInt\cite{lindell2021_autoint_cvpr21}                    & \textcolor{blue}{4.5}           & -----                   & 3.16                                                     & -----                                                        & -----                                                          & 18.6                          & 24.14                      \\
            NeX\cite{wizadwongsa2021nex}                                & 89.0           & 42.7     & \textbf{120.05}                                          & -----                                                        & -----                                                          & \textbf{706.1}                & 27.26                      \\
            TermiNeRF-8\cite{piala2021terminerf}                        & \textcolor{orange}{4.1}         & -----                   & 2.30                                                     & -----                                                        & 21.4*                                                          & 13.5 - 15.1                & 23.02                      \\
            RSEN\cite{attal2021learning}                                & 5.4                           & 67.2     & 4.79                                                     & -----                                                        & -----                                                          & 28.2                          & \textbf{27.94}             \\
            AdaNeRF\cite{kurz2022adanerf}                               & \textcolor{orange}{4.1}          & \textcolor{blue}{7.6}     & -----                                                    & -----                                                        & 41.0*                                                          & 30.3                          & 25.10                      \\
            R2L\cite{wang2022r2l} (88-layer)                            & 23.7                          & 11.8                   & 3.65                                                     & 4.73                                                         & -----                                                          & 18.9 - 21.4                   & \textcolor{orange}{27.79}     \\
            R2L\cite{wang2022r2l} (16-layer)                            & 4.6                          & \textcolor{orange}{2.4}   & \textcolor{blue}{16.67}                                   & 20.12                                                        & -----                                                          & \textcolor{blue}{80.5 - 98.1}& 24.42                      \\
            \midrule
            NeRDF-D8G8 (Ours)                                           & 5.1                  & 2.6           & \textcolor{orange}{16.80}                                  & 22.37                                                         & -----                                                          & \textcolor{orange}{89.5 - 98.8}        & 26.53                      \\ \bottomrule
            \end{tabular}
    }
\end{table*}
